Personalized Filled-pause Generation with Group-wise Prediction Models

In this paper, we propose a method to generate personalized filled pauses (FPs) with group-wise prediction models. Compared with fluent text generation, disfluent text generation has not been widely explored. To generate more human-like texts, we addressed disfluent text generation. The usage of disfluency, such as FPs, rephrases, and word fragments, differs from speaker to speaker, and thus, the generation of personalized FPs is required. However, it is difficult to predict them because of the sparsity of position and the frequency difference between more and less frequently used FPs. Moreover, it is sometimes difficult to adapt FP prediction models to each speaker because of the large variation of the tendency within each speaker. To address these issues, we propose a method to build group-dependent prediction models by grouping speakers on the basis of their tendency to use FPs. This method does not require a large amount of data and time to train each speaker model. We further introduce a loss function and a word embedding model suitable for FP prediction. Our experimental results demonstrate that group-dependent models can predict FPs with higher scores than a non-personalized one and the introduced loss function and word embedding model improve the prediction performance.

==> tex/exp_ver1.tex <==
\section{Experiment} \label{sec:exp}
To evaluate the prediction accuracy of models for FP's positions and words, we used precision, recall, F-score, and specificity. First, for positions, precision was defined as the rate of positions actually having FPs out of those predicted to have FPs, and recall was defined as the rate of positions predicted to have FPs out of those actually having FPs, and F-score was calculated from these scores. The specificity was the rate of positions predicted to have no FPs out of the positions actually having no FPs. For each FP's word, we calculated precision, recall, F-score, and specificity in the same way. As the score of the prediction accuracy for FP words, we used the average of each word's score weighted by the frequency of each FP.
    
    % Exp 0: open / close
    \subsection{Preliminary evaluation} \label{ssec:exp_open_close}
        In order to investigate whether the general model is effective for unseen speakers (i.e. speakers not included in the training data), we compared the prediction accuracy for speakers included and not included in the training data.
    
        \subsubsection{Experimental setting} \label{sssec:exp_setting_open_close}
            The data of $137$ speakers from the CSJ was used, and the data of $100$ speakers of them was split into training data, validation data, and test data so that the data of each speaker was included in all the sets in a ratio of approximately 3:1:1 (speaker-closed). The prediction accuracy of the test data was compared with the prediction accuracy of all the data of the remaining $37$~speakers (speaker-opened). In this paper, we used the breath paragraph separated by a silence for $0.2$~seconds or longer as the utterance unit. Sudachi~\cite{takaoka18sudachi} was used for morphological analysis. In this experiment, the word embedding model was fastText, which had been pre-trained on large-scale Japanese data, and the embedding dimension was set to $300$\footnote{\url{https://fasttext.cc/docs/en/crawl-vectors.html}}. We set the number of hidden layers to $1$, hidden size to $1024$, and dropout probability to $0.0$. Adam was used as the optimizer and the gradient clipping was applied. The size of batches is $32$. These were applied below unless otherwise stated. The learning rate was set to 1.0×\( 10^{-3} \), multiplied by $0.1$ every $40$~epochs, and the model was trained for $200000$~steps.
        
        \subsubsection{Result} \label{sssec:exp_result_open_close}
            Table~\ref{tab:open_close} show that the speaker-closed prediction has higher values except for the precision for predicting position, indicating that the speaker-closed prediction is more accurate than the speaker-opened prediction for both position and word. However, since the difference between the speaker-closed and speaker-opened scores is only about $0.04$ in the F-score, the speaker-opened prediction can be used sufficiently. Therefore, the general model can be used to predict FPs of unseen speaker when it is not important to predict the personalized FPs, but the generalized FPs are required. The value of specificity is close to $1.0$, indicating that FPs are rarely inserted in positions where there are actually no FPs. This is also true for the other results.
            
            Based on the above results, which show that speaker-opened prediction can provide sufficient accuracy compared to speaker-closed one, we conducted the cross validation in the following evaluation of prediction accuracy.
            
            \input{tab/open_close}
    
    % Exp 1: Weighted cross entropy loss
    \subsection{Weighted cross entropy loss}
    \label{ssec:exp_weighted_loss}
    
        \subsubsection{Experimental setting} \label{sssec:exp_setting_weighted}
            The data of $137$~speakers from the CSJ was used. For the prediction model, fastText and BLSTM were used as in Section~\ref{ssec:exp_open_close}. The learning rate was multiplied by $0.1$ every $50000$~steps, and the other hyper-parameters were same as in Section~\ref{ssec:exp_open_close}. To evaluate the accuracy of models, cross validation was applied. The speakers were divided into $10$~sets. Then, models were trained using $9$ of these sets as training data, and the remaining set was used for evaluation. The average of the evaluation scores obtained by repeating this process $10$~times was the evaluation score of the general model. The missed scores was considered as $0.0$, and the average score was calculated.
        
        \subsubsection{Result} \label{sssec:exp_result_weighted}
            Table~\ref{tab:weighted_loss} shows that the F-score, which is an criterion that takes into account both precision and recall, is higher for both positions and words when weights are used, indicating that the using loss weights improved the prediction accuracy of positions and words. The precision of the model with weights is lower and the recall of that is higher for both positions and words. This indicates that introducing the weights makes the model actively insert FPs and improves the recalls, but it increases the number of mistakes. This is consistent with the result that the position's specificity is decreasing.
            
            Based on this result, we used weighted cross entropy loss in the following experiments.
            
            \input{tab/weighted_loss}
    
    % Exp 2: BERT
    \subsection{Rich word embedding model} \label{ssec:exp_bert}
    
        \subsubsection{Experimental setting} \label{sssec:exp_setting_bert}
            The same data and fastText model were used as in Section~\ref{ssec:exp_weighted_loss}, and the texts were segmented to morphemes by Juman++~\cite{morita15jumanpp} to use as the inputs of the BERT model. We used the model that has been trained on a large-scale Japanese data published by the Kurohashi-Chu-Murawaki labs at Kyoto University\footnote{\url{https://nlp.ist.i.kyoto-u.ac.jp/?ku_bert_japanese}}. The version of the model was the LARGE WWM. The learning rate was set to 1.0×\( 10^{-5} \) and models were trained for $60000$~steps. To evaluate the prediction accuracy, the cross validation with $10$~partitions was performed as in Section~\ref{ssec:exp_weighted_loss}.
        
        \subsubsection{Result} \label{sssec:exp_result_bert}
            Table~\ref{tab:fasttext_bert} shows that BERT has a higher value than fastText except for position's recall and word's specificity, which indicates that the prediction accuracy is improved by using BERT as a word embedding model.
            
            Based on this result, BERT was used as the word embedding model in the following experiments.
            
            \input{tab/fasttext_bert}
    
    % Exp 3: Positional encoding
    % \subsection{Positional encoding} \label{ssec:exp_pos_enc}
    
    %     \subsubsection{Experimental setting} \label{sssec:exp_setting_pos_enc}
    %         transformer[引用]で用いられている，sin,cos関数によるpositional encodingを用いる．BLSTMの出力に，positional embeddingを足し合わせる．学習率は1.0×10^-5とし，60000step学習させたモデルを用いる．予測精度の評価には，これまでと同様に分割数10の cross validation を行う．
            
    %         \subsubsection{Result} \label{sssec:exp_result_pos_enc}
    %         表~を見ると，位置のF scoreはほぼ等しく，種類のF scoreはpositional encodingを用いた方が高くなっている．また，positional encodingを用いた方が，位置・種類ともにprecisionが低くrecallが高い値となっている．これらから，positional encodingにより種類の予測精度を向上させることが可能で，また少し正解率は犠牲となるが積極的なフィラーの挿入が可能となる．
            
    %         あとで cross validation の結果に差し替え
    %         \input{tab/pos_enc}
    
    % Exp 4: 話者適応とグルーピング
    \subsection{Constructing group-dependent prediction model} \label{ssec:exp_group}
    
        \subsubsection{Experimental setting} \label{sssec:exp_setting_group}
            We describe the method of grouping speakers. In order to deal with the sparsity of FP positions and the bias of FP words, the hierarchical clustering was performed based on the trends of FP positions and words.
            First, for clustering by the usage of FP word, the rate of the usage of each FP word was calculated by dividing the number of each FP word usage by the total number of FP usage for each speaker. Then, hierarchical clustering was applied using Euclidean distance and Ward's method. With the distance threshold set to $1.0$, the speakers were classified into four classes based on the distance.
            Next, for clustering by positional tendency, we use 1) head of sentence, 2) intra-sentence and boundary of breath paragraph, 3) intra-sentence and middle of breath paragraph, and 4) end of sentence as FP positions, and the rate of each FP position usage was calculated by dividing the number of each FP position usage by the total number of FPs for each speaker. Then, the hierarchical clustering was applied using Euclidean distance and Ward's method. With the distance threshold set to $1.7$, the speakers were classified into four classes based on the distance.
            
            \textbf{General model.} 
            The data of $137$ speakers from the CSJ was used, the learning rate was set to 1.0×\( 10^{-5} \), and the model was trained for $60000$ steps. To evaluate the prediction accuracy, the cross validation with $10$ partitions was performed as in Section~\ref{ssec:exp_weighted_loss}.
            
            \textbf{Group-dependent model.} 
            Group-dependent models were constructed by fine-tuning the general model using data from each of the four classes clustered by the trends of positions and words. The learning rate was set to 1.0×\( 10^{-5} \), and the models were trained for $10000$~steps. To evaluate the prediction accuracy, the cross validation was performed as before. Since the number of data in each group was smaller than before, the number of speaker partitions was set to $5$.
            
            \textbf{Speaker-dependent model.} 
            As described in Section~\ref{ssec:method_group}, we used the lecture data of the University of Tokyo available on Youtube\footnote{\url{https://youtube.com/playlist?list=PLHxBhbJJasnfX6oBrkTygP8we61wEcRha}} for two speakers. Each speaker's data was divided into train data, validation data, and test data. The speaker-dependent models were trained for $10000$~steps with a learning rate of 1.0×\( 10^{-5} \) by fine-tuning the general model trained for $60000$~steps. The test data was used to evaluate the accuracy of the models.
        
        \subsubsection{Result of clustering} \label{sssec:exp_result_clustering}
            Figure~\ref{fig:clustering_word} shows the results of calculating the each FP word's rate for each class by FP words. Cluster~1, 2, 3, and 4 contain $18$, $55$, $25$, and $39$~speakers respectively. Cluster~2, 3, and 4 have a high usage rate of "ee"; "ano", "anoo"; "ma", "maa", whereas Cluster~1 has a high usage rate of "ee", and FPs other than "ee" and "e" were rarely used.
            Figure~\ref{fig:clustering_position} shows the results of calculating the each FP position's rate for each class by FP positions. Cluster~1, 2, 3, and 4 contain $50$, $13$, $27$, $47$~speakers respectively. FPs are used more frequently at the middle of breath paragraph in Cluster~1, at the head of sentences in Cluster~2, at the beginning of breath paragraph in Cluster~3, whereas Cluster~4 shows an average tendency among all classes.
            
            \input{fig/class}
        
        \subsubsection{Evaluation of group-dependent models} \label{sssec:exp_result_group}
            Table~\ref{tab:class_word} shows the prediction accuracy of the general model and the group-dependent models by FP word's tendency, indicating that the prediction accuracy of all group-dependent models is higher than that of the general model for both positions and words. Therefore, the grouping of speakers by FP words proposed in this paper improves the accuracy. 
            And then, Table~\ref{tab:class_position} shows the prediction accuracy of the general model and the group-dependent models by FP position's tendency, indicating that the prediction accuracy of the group-dependent models is higher than that of the general model, except for the position's F-score of the Cluster~2. Therefore, the grouping of speakers by FP position's tendency proposed in this paper improves the accuracy for almost all groups.
            Moreover, Table~\ref{tab:speaker_model} shows the prediction accuracy of the speaker-dependent model. Speaker-dependent models have the lowest accuracy for both speakers, indicating that it is difficult to adapt the prediction model to speakers.
            
            \input{tab/class}

        \subsubsection{Evaluation of prediction for each FP} \label{sssec:exp_result_eachfp}
            Figure~\ref{fig:each_FP} shows the prediction accuracy of each FP word in the group-dependent model by FP word's tendency, and that in the group-dependent model by FP position's tendency. The horizontal axis expresses FP words, and the more on the right, the less frequent in the corpus. The models for word's Cluster~2, position's Cluster~1 and 4 are more accurate than the general model for all FP words. In contrast to the general model which is more accurate for highly frequent FPs but less accurate for less frequent ones, the above models have prediction accuracy for less frequent FPs close to that of frequent FPs. The models for word's Cluster~3 and 4, and position's Cluster~3 are more accurate than the general model for FPs other than "ee", and the accuracy for less frequent FPs are high. The model for word's Cluster~1 is less accurate than the general model for some FPs. In addition, the position's Cluster~2 model has a low prediction accuracy of 0 for about half of the FPs.
            
            \input{fig/class_each_filler}
        
        \subsubsection{Evaluation of predictions for each speaker} \label{sssec:exp_result_eachspk}
            We describe the distribution of each speaker's prediction accuracy by the group-dependent models. The cross validation was not performed, but the data was divided into training data, validation data, and test data in an approximate ratio of 3:1:1 under the speaker-closed condition, and the results was evaluated using the test data. The results are shown in Figure~\ref{fig:each_spk}. The F-scores for each cluster of positions and words are widely distributed, indicating that grouping speakers improves the prediction accuracy on average, but the tendency of improvement differs from speaker to speaker.
            
            \input{fig/class_each_speaker}
        
        \subsubsection{Evaluation on lecture data} \label{sssec:exp_result_lec}
            We compared the prediction accuracy of the general, group-dependent, and speaker-dependent models on the test data of lectures described in Section~\ref{sssec:exp_setting_group}. The results are shown in Table~\ref{tab:speaker_a}. The results for speaker~A show that the accuracy of the general model is the highest, followed by the speaker-dependent model, and the group-dependent models have the lowest accuracy. Speaker~B shows the same results in Table~\ref{tab:speaker_b}.
            The results for speaker~B show that the accuracy of the general model is the highest, followed by the group-dependent models, and the speaker-dependent model has the lowest accuracy.
            
            \input{tab/speaker}
        
        \subsubsection{Discussion} \label{sssec:exp_discuss}
            The experimental results demonstrated that grouping speakers based on their FPs' usage enabled the construction of group-dependent models with higher prediction accuracy than the general model. The one possible reason for this is that grouping by FP usage reduces the variation in usage tendency within the data group, which makes the model training easier. Another possible reason is that the difference in tendency between the training and evaluation data is reduced. This is an effective result because the prediction model of data group close to target speaker's data is actually used for predicting unseen speakers.
            
            In the evaluation using the lecture data, the accuracy of the general model was the highest. Considering the results in Figure~\ref{fig:each_spk}, which show that the accuracy of the prediction models differed among speakers, this suggests that the two speakers used in this experiment have particularly low prediction accuracy. Since the CSJ consisting mainly of conference presentations was used for general and group-dependent training, while the lecture data by the lecturer was used for evaluation, such difference of the domains between the spontaneous speech data is also a possible reason for the above results.
